Robust Finite-State Controllers for Uncertain POMDPs

Uncertain partially observable Markov decision processes (uPOMDPs) allow the probabilistic transition and observation functions of standard POMDPs to belong to a so-called uncertainty set. Such uncertainty, referred to as epistemic uncertainty, captures uncountable sets of probability distributions caused by, for instance, a lack of data available. We develop an algorithm to compute finite-memory policies for uPOMDPs that robustly satisfy specifications against any admissible distribution. In general, computing such policies is theoretically and practically intractable. We provide an efficient solution to this problem in four steps. (1) We state the underlying problem as a nonconvex optimization problem with infinitely many constraints. (2) A dedicated dualization scheme yields a dual problem that is still nonconvex but has finitely many constraints. (3) We linearize this dual problem and (4) solve the resulting finite linear program to obtain locally optimal solutions to the original problem. The resulting problem formulation is exponentially smaller than those resulting from existing methods. We demonstrate the applicability of our algorithm using large instances of an aircraft collision-avoidance scenario and a novel spacecraft motion planning case study.

==> flowchart_problem.tex <==
\definecolor{bg}{HTML}{ddeedd}
\definecolor{comp}{HTML}{c2d4dd}
\definecolor{impl}{HTML}{b0aac0}
\definecolor{ligb}{HTML}{5E7FC6}
\definecolor{bodybl}{HTML}{85A1DC}
\definecolor{headbl}{HTML}{264C9C}
\definecolor{bgyel}{HTML}{FFDC6B}
\definecolor{bodyyel}{HTML}{FFE58F}
\definecolor{headyel}{HTML}{E9BB25}
%
\centering
\begin{tikzpicture}[every node/.style={draw, text centered, shape=rectangle, rounded corners, text width=3cm, minimum height=1.3cm, inner sep=3pt}, blank/.style={draw=none,fill=none,ultra thick,inner sep=0.001pt}]
%\tikzstyle{outer}= [draw, text centered, shape=rectangle, text width=2cm, minimum height=1cm]
%\tikzstyle{inner}=[draw, text centered, shape=rectangle, rounded corners, text width=3.8cm, minimum height=1.1cm, inner sep=5pt]
\tikzset{
	splitnode/.style={
		rectangle split,
		rectangle split parts=2,
		rectangle split part fill={headbl!70,bodybl!60}
	}
}
\tikzset{
	normalnode/.style={
		fill=red!10
	}
}
\tikzstyle{split}=[rectangle split,rectangle split parts=2]


%\node[splitnode](lp) {\textbf{Local Improvement} \nodepart{second} Linear Program for each $s\in S'$};
%\node[splitnode,right=1.0cm of lp] (newsamp) {\textbf{Training Data} \nodepart{second} POMDP Observation-Action Sequences};
%\node[normalnode, below=0.5cm of newsamp] (drnn) {\textbf{Recurrent\\Neural Network}};
%\node[splitnode, below=0.5cm of newsamp] (strategy) {\textbf{Strategy} \nodepart{second} Strategy $\osched$ for $\pomdp$};


\node[normalnode] (infinite-qcqp) {\textbf{Semi-infinite \linebreak Nonconvex Problem} %\nodepart{second} DTMC $\pomdp^\osched$
};

\node[normalnode, above=1.5cm of infinite-qcqp] (infinite-convex-qcqp) {\textbf{Finite\linebreak Nonconvex Problem} 
%	\nodepart{second} $\pomdp^\sigma\models\reachPropSymbol$~?
};
%\node[splitnode,above=1.5cm of model](count) {\textbf{Counterexamples} \nodepart{second} Set $S'\subseteq S$ of critical states};
\node[normalnode, right=2.3 cm of infinite-convex-qcqp] (finite-qcqp) {\textbf{Finite LP}}; %\nodepart{second} DTMC $\pomdp^\osched$

%\node[splitnode, right=2 cm of finite-qcqp] (strategy) {\textbf{Strategy}\nodepart{second}Strategy  $\sched$ for $\pomdp$};

\node[splitnode, below=1.5 cm of finite-qcqp] (verification) {\textbf{Robust Verification}\nodepart{second} Verifying uMC $\pomdp^{\sched} \models \varphi$};

\draw (finite-qcqp) edge[-latex', very thick] (verification);
      \node[blank,above right=-2.65cm and -4.0cm of finite-qcqp] {\textbf{Solve \linebreak LP\\(Section~\ref{sec:scp})}};
%\node[text width=2.5cm,minimum height=1.3cm,draw=none,right=1.7cm of newsamp] (drnn) {\textbf{Recurrent\\Neural Network}\vspace{6pt} \includegraphics[width=0.8\textwidth]{pics/layer_icon}};

\draw (infinite-qcqp) edge[-latex', very thick] (infinite-convex-qcqp);
\node[blank,above right=-2.55cm and -2.2cm of infinite-convex-qcqp] {\textbf{Dualize\\(Section~\ref{sec:uncertainty})}};

\draw (infinite-convex-qcqp) edge[-latex', very thick] (finite-qcqp);

      \node[blank,above right=-0.7cm and -0.45cm of infinite-convex-qcqp] {\textbf{ Linearize \\Around $\sched$ \\ (Section~\ref{sec:scp}) }};

%\begin{scope}[on background layer]
%\node [fit = (current bounding box), inner sep = .1cm,  fill=bodyyel] (box) {};
%\end{scope}

%\node[splitnode, right=2.65cm of drnn] (trajsamp) {\textbf{Trajectory Samples} \nodepart{second} For entire problem class};

%\node[normalnode, below=1cm of model, minimum height=1cm, text width=2cm] (spec) {\textbf{Specification}};

\node[splitnode, below=0.6cm of infinite-qcqp] (pomdp) {\textbf{Uncertain Model} \nodepart{second}uPOMDP $\pomdp$ \\ Specification $\varphi$};

\node[draw=none,below=1.2cm of verification,minimum height=0.1cm,text width =0.5cm] (safe) {\color{green!70!black}\Large\checkmark};


%%arrows
%\draw ([yshift=-2ex] testing.west) edge[-latex', very thick] ([yshift=-2ex] system.east);
%\draw ([yshift=2ex] system.east) edge[-latex', very thick] ([yshift=2ex] testing.west);

%\path [-latex', very thick, dashed] (model) --node[draw=none,left,text width=1.2cm]{\small UNSAT } (count);
\path [-latex', very thick, dashed] (verification) --node[draw=none,left=0.5cm,text width=0.25cm,minimum height=0.05cm]{\textbf {SAT}} (safe);

\draw (pomdp) edge[-latex', very thick] (infinite-qcqp);

\draw (verification) edge[-latex', very thick, dashed] (safe);
\draw (verification) edge[-latex', very thick, dashed] (infinite-qcqp);

      \node[blank,above right=-1.4cm and -0.4cm of infinite-qcqp] {\textbf{ UNSAT \linebreak\linebreak {Update $\sched$}}};
%\draw (newsamp) edge[-latex', very thick] (drnn);

%\draw (newsamp.south) edge[-latex', very thick] (strategy.north);

%\draw (strategy.south) edge[-latex', very thick] (dtmc.north);

%\draw (dtmc.west) edge[-latex', very thick] (model.east);

%\draw (pomdp) edge[-latex', very thick] (dtmc);
%\draw (pomdp) edge[-latex', very thick] (trajsamp);
%\draw (trajsamp) edge[-latex', very thick] (drnn);
\end{tikzpicture}


==> grid.tex <==
\begin{tikzpicture}
    [%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        box/.style={rectangle,draw=black,thick, minimum size=1cm},
    ]%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\foreach \x in {0,1,...,4}{
    \foreach \y in {0,1,...,4}
        \node[box] at (\x,\y){};
}
\colorlet{darkgreen}{green!50!black}
\node[box,fill=darkgreen] at (4,4){};  
\node[box,fill=red  ] at (3,3){};  
\node[box,fill=red ] at (3,1){};
\node[box,fill=red ] at (1,4){};
%\node[draw=white] at (6,4){};
	\draw[thick,blue,->] (1.0,1.0) -- (1,2);
		\draw[thick,blue,->] (1.0,1.0) -- (1,0);
	\draw[thick,blue,->] (1.0,1.0) -- (0,1);

	\draw[thick,blue,->] (1.0,1.0) -- (2,1);

\draw (1.00, 1.00) node[inner sep=0] {\includegraphics[width=.041\textwidth]{pics/Robot.png}};
\end{tikzpicture}


==> maze.tex <==
\begin{tikzpicture}
    [%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        box/.style={rectangle,draw=black,thick, minimum size=1cm},
    ]%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\colorlet{darkgreen}{green!70!black}


        \node[box] at (0,0){};
        \node[box] at (1,0){};
        \node[box] at (2,0){};
        \node[box] at (3,0){};
        \node[box] at (4,0){};
        \node[box] at (4,-1){};
        \node[box] at (4,-2){};
        \node[box] at (4,-3){};
        \node[box] at (2,-1){};
        \node[box] at (2,-2){};
        \node[box] at (2,-3){};

        \node[box] at (0,-1){};
        \node[box] at (0,-2){};
        \node[box] at (0,-3){};

  \node [draw=none] at (0,0) {\Huge $0$};
  \node [draw=none] at (1,0) {\Huge $1$};
  \node [draw=none] at (2,0) {\Huge $2$};
  \node [draw=none] at (3,0) {\Huge $3$};
  \node [draw=none] at (4,0) {\Huge $4$};
    \node [draw=none] at (0,-1) {\Huge $5$};
    \node [draw=none] at (2,-1) {\Huge $6$};
    \node [draw=none] at (4,-1) {\Huge $7$};
    \node [draw=none] at (0,-2) {\Huge $8$};
    \node [draw=none] at (4,-2) {\Huge $9$};
    \node [draw=none] at (2,-2) {\Huge ${10}$};
    \node [draw=none] at (0,-3) {\Huge $11$};
    \node [draw=none] at (4,-3) {\Huge $12$};
    \node [draw=none] at (2,-3) {\Huge ${\color{darkgreen}13}$};




\end{tikzpicture}


==> pics/macros.tex <==
%% Commands requiring trailing spaces
\DeclareMathOperator*{\argmin}{argmin} 

\newcommand{\ie}{i.e.\@\xspace}
\newcommand{\wrt}{w.r.t.\@\xspace}
\newcommand{\eg}{e.g.\@\xspace}
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\etal}{\emph{et al.}\@\xspace}
\newcommand{\prophesy}{\textrm{PROPhESY}\xspace}
\newcommand{\prism}{\textrm{PRISM}\xspace}
\newcommand{\storm}{\textrm{Storm}\xspace}
\newcommand{\tool}[1]{\textrm{#1}\xspace}


%%new commands
\newcommand{\dtmc}{\mathcal{D}}
\newcommand{\dtmcInit}[1][]{\ensuremath{\dtmc{#1}=(S{#1},\sinit{#1},P{#1})}}
\newcommand{\p}{\ensuremath{\mathbb{P}}}
\newcommand{\pr}{\ensuremath{\mathrm{Pr}}}
\newcommand{\reachPr}[2]{\ensuremath{\pr^{#1}(\finally #2)}}
\newcommand{\reachPrT}[1][]{\ensuremath{\reachPr{#1}{T}}}
\newcommand{\reachProp}[2]{\ensuremath{\p_{\leq #1}(\finally #2)}}
\newcommand{\reachProplT}{\ensuremath{\reachProp{\lambda}{T}}}
\newcommand{\reachPrs}[3]{\ensuremath{\pr^{#1}_{#2}(\finally #3)}}
%\newcommand{\reachPrsT}[2]{\ensuremath{\reachPrs{#1}{#2}{T}}}
\newcommand{\reachPropSymbol}{\varphi}
\newcommand{\ereachPropSymbol}{\psi}

\newcommand{\rew}{\ensuremath{r}}
\newcommand{\er}{\ensuremath{\mathrm{ER}}}
\newcommand{\expRew}[2]{\ensuremath{\er^{#1}(\finally #2)}}
\newcommand{\expRewT}[1][]{\ensuremath{\expRew{#1}{T}}}
\newcommand{\expRewProp}[2]{\ensuremath{\er_{\leq #1}(\finally #2)}}
\newcommand{\expRewPropkT}{\ensuremath{\expRewProp{\kappa}{T}}}
\newcommand{\rewFunction}{\ensuremath{\mathrm{rew}}}
\newcommand{\finally}{\lozenge}


\newcommand{\creachPr}[3]{\ensuremath{\pr^{#1}(\finally #2 \mathrel{|} \neg \finally #3)}}
\newcommand{\creachPrT}[1][]{\ensuremath{\creachPr{#1}{T}{U}}}
\newcommand{\creachProp}[3]{\ensuremath{\p_{\leq #1}(\finally #2 \mathrel{|} \neg \finally #3)}}
\newcommand{\creachProplT}{\ensuremath{\creachProp{\lambda}{T}{U}}}
\newcommand{\creachPrs}[4]{\ensuremath{\pr^{#1}_{#2}(\finally #3 \mathrel{|} #4)}}

\newcommand{\cexpRew}[3]{\ensuremath{\er^{#1}(\finally #2 \mathrel{|} \neg \finally #3)}}
\newcommand{\cexpRewT}[1][]{\ensuremath{\cexpRew{#1}{T}{U}}}

\newcommand{\cexpRewProp}[3]{\ensuremath{\rew_{\leq #1}(\finally #2 \mathrel{|} \neg \finally #3)}}
\newcommand{\cexpRewPropkT}{\ensuremath{\cexpRewProp{\kappa}{T}{U}}}



%% Comments
\newcommand{\commentside}[2]{\marginpar{\color{#1}\tiny#2}}
\newcommand{\TODO}[1]{\commentside{teal}{\textsc{Todo:} #1}}
\newcommand{\REMARK}[1]{\commentside{teal}{\textsc{Remark:} #1}}
\newcommand{\nj}[1]{\todo[inline,color=yellow!50]{\color{black}NJ: #1}\color{black}}
\newcommand{\lmc}[1]{\todo[inline,color=green!50]{\color{black}MC: #1}\color{black}}
%\newcommand{\njs}[1]{\commentside{yellow!70!black}{NJ: #1}}
\newcommand{\bk}[1]{\todo[inline,color=red!40]{BK: #1}}
%\newcommand{\bkss}[1]{\todo[color=red!40]{BK: #1}}
%\newcommand{\bks}[1]{\commentside{red!40}{BK: #1}}
\newcommand{\cd}[1]{\todo[inline,color=blue!40]{\color{black}CD: #1}\color{black}}
%\newcommand{\fos}[1]{\commentside{blue!40}{FO: #1}}
\newcommand{\lw}[1]{\todo[inline,color=green!70!black]{\color{black}LW: #1}\color{black}}
%\newcommand{\fgs}[1]{\commentside{green!70!black}{FG: #1}}
\newcommand{\jpk}[1]{\todo[inline,color=orange]{\color{white}JPK: #1}\color{black}}
%\newcommand{\jpks}[1]{\commentside{orange}{JPK: #1}}



%% Sets
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\Reals}{\ensuremath{\mathbb{R}}\xspace}    % Real numbers
\newcommand{\Rationals}{\ensuremath{\mathbb{Q}}\xspace}    %Rational numbers
\newcommand{\Integers}{\ensuremath{\mathbb{Z}}\xspace}    %Integer numbers
\newcommand{\Naturals}{\ensuremath{\mathbb{N}}}
\newcommand{\Ireal}{[0,\, 1]\subseteq\mathbb{R}}  % real interval [0,1]
\newcommand{\Irat}{[0,\, 1]\subseteq\mathbb{Q}}  % rational interval [0,1]
\newcommand{\Ex}{\ensuremath{\mathbb{E}}\xspace}        % Expectations
\newcommand{\BEx}{\ensuremath{\mathbb{E}_{\scriptscriptstyle \leq 1}}\xspace}        % Expectations
\newcommand{\ExCPO}{\ensuremath{\mathcal{E}}\xspace}              % Cpo of unbounded expectations
\newcommand{\BExCPO}{\ensuremath{\mathcal{E}_{\leq 1}}\xspace}        % Cpo of bounded expectations
\newcommand{\EV}{\ensuremath{\mathbf{E}}}

\newcommand{\Distr}{\mathit{Distr}}
\newcommand{\subDistr}{\mathit{subDistr}}
\newcommand{\distDom}{X}
\newcommand{\distDomFin}{\DistDom=\{x_1,\, \ldots,\, x_n}
\newcommand{\distFunc}{\mu}
\newcommand{\distDomElem}{x}
\newcommand{\supp}{\mathit{supp}}
\newcommand{\bigland}{\ensuremath{\bigwedge}}
\newcommand{\biglor}{\ensuremath{\bigvee}}


%% Constants
\newcommand{\true}{\ensuremath{\mathsf{true}}\xspace}
\newcommand{\false}{\ensuremath{\mathsf{false}}\xspace}
\newcommand{\ExpZero}{\CteFun{0}\xspace}
\newcommand{\ExpOne}{\CteFun{1}\xspace}


%% Math operators
\newcommand{\dual}[1]{{#1}^{\mathcal{D}}\xspace}               % Dual 
\newcommand{\eqdef}{\triangleq}                              % Equality used for definitions
\DeclareMathOperator*{\lfp}{\boldsymbol \mu}            % Least fixed point
\DeclareMathOperator*{\gfp}{\boldsymbol \nu}            % Greatest fixed point
\newcommand{\suchthat}{\mydot}
\newcommand{\dom}{\ensuremath{\mathit{dom}}}

\newcommand{\mydot}{\ensuremath                         % Scope delimiter (eg forall, lambda abstractions)
  \raisebox{0pt}{${\scriptscriptstyle \bullet}~$}}
\newcommand{\CteFun}[1]{\ensuremath{\boldsymbol{#1}}\xspace}    % Constant function


%% Linear temporal logic
\newcommand{\Always}{\Box \, }
\newcommand{\Finally}{\lozenge \, }
\newcommand{\Ever}{\Diamond \, }
\newcommand{\Next}{\bigcirc \, }
\newcommand{\Until}{\mbox{$\, {\sf U}\,$}}
\newcommand{\Unless}{\mbox{$\, {\sf W}\,$}}


%% Program Semantics
\renewcommand{\wp}{{\sf wp}\xspace}
\newcommand{\wlp}{{\sf wlp}\xspace}
\newcommand{\wllp}{{\textsf{w}(\textsf{l})\textsf{p}}\xspace}
\newcommand{\cwp}{{\sf cwp}\xspace}
\newcommand{\cwlp}{{\sf cwlp}\xspace}
\newcommand{\cwllp}{{\textsf{cw}(\textsf{l})\textsf{p}}\xspace}
\newcommand{\qcwp}{\ensuremath{\mathsf{\ushortw{cw}p}}\xspace}
\newcommand{\qcwlp}{\ensuremath{\mathsf{\ushortw{cwl}p}}\xspace}
%\newcommand{\qcwllp}{\ensuremath{\mathsf{\ushortw{cw\textnormal{(}l\textnormal{)}}p}}\xspace}
\newcommand{\sem}[1]{\llbracket #1 \rrbracket}
\newcommand{\ToExp}[1]{\ensuremath{ \chi_{#1} }\xspace}    % Lifting of predicates into expectations
%\newcommand{\ToExp}[1]{\ensuremath{\left[ #1 \right]}\xspace}    % Lifting of predicat
 \newcommand{\Pre}{\Psi}
 \newcommand{\Post}{\Phi}
% \newcommand{\Inv}{\Theta}


%% pGCL LANGUAGE
\newcommand{\GCL}{\textnormal{\textsf{GCL}}\xspace}
\newcommand{\pGCL}{\textnormal{\textsf{pGCL}}\xspace}
\newcommand{\fpGCL}{\textnormal{$\textsf{pGCL}^{\boxtimes}$}\xspace}
\newcommand{\cpGCL}{\textnormal{\textsf{cpGCL}}\xspace}
\newcommand{\cfpGCL}{\textnormal{$\textsf{cpGCL}^{\boxtimes}$}\xspace}
%%% Set of variables,states,expressions,etc  
\newcommand{\Cmd}{\ensuremath{\mathcal{P}}\xspace}        % Set of programs
\newcommand{\Var}{\ensuremath{\mathcal{V}}\xspace}        % Set of program variables 
\newcommand{\Paramvar}{\ensuremath{{V}}\xspace}        % Set of program variables 

\newcommand{\RExpr}{\ensuremath{\mathcal{E}}\xspace}      % Set of arithmetical expressions   
\newcommand{\BExpr}{\ensuremath{\mathcal{B}}\xspace}      % Set of boolean expressions
\newcommand{\PDom}{\ensuremath{\mathfrak{P}}\xspace}
%\newcommand{\State}{\ensuremath{\mathbb{S}}\xspace}      
\newcommand{\Loop}{\textsf{loop}\xspace} % shorthand to talk about loops
\newcommand{\Body}{\textsf{body}\xspace}
\newcommand{\Init}{\textsf{init}\xspace}
\newcommand{\counter}{\textit{cntr}\xspace}
\newcommand{\intercepted}{\textit{int}\xspace}
\newcommand{\delivered}{\textit{del}\xspace}
\newcommand{\continue}{\textit{rerun}\xspace}
%%% Language constructs
\newcommand{\Skip}{{\tt skip}\xspace}
\newcommand{\Abort}{{\tt abort}\xspace}
\newcommand{\Ass}[2]{#1 \coloneqq #2}
\newcommand{\Observe}{\textnormal{\texttt{observe}}\xspace}
\newcommand{\PChoice}[3]{\{#1\} \, \left[#2 \right] \, \{#3\}}
\newcommand{\NDChoice}[2]{\{#1\} \, \Box \, \{#2\}}
\newcommand{\If}{{\tt if}\xspace}
\newcommand{\Then}{{\tt then}\xspace}
\newcommand{\Else}{{\tt else}\xspace}
\newcommand{\While}{{\tt while}\xspace}
\newcommand{\For}{{\tt while}\xspace}

\newcommand{\Do}{{\tt do}\xspace}
\newcommand{\Ite}{{\tt ite}\xspace}
\newcommand{\Cond}[3]{{\Ite} \, (#1) \allowbreak\, \{#2\} \allowbreak\, \{#3\}}
\newcommand{\WhileDo}[2]{{\While} \,\allowbreak (#1) \,\allowbreak \{#2\}}
\newcommand{\WhileDok}[3]{{\While}^{{}< #1} \,\allowbreak (#2) \,\allowbreak \{#3\}}
\newcommand{\Assert}{{\sf assert}\xspace}


%% Miscellania 
\newcommand{\Tr}{\ensuremath{\mathcal{T}}}    % Program transformation
\newcommand{\To}{\rightarrow}                          % Function space constructor
\newcommand{\subst}[2]{[#1 / #2]}
\newcommand{\ourunderscore}{\rule{1.5ex}{0.4pt}}


%% Operational Semantics
\newcommand{\sinit}{s_{\mathit{I}}} % initial state of DTMC/MDP
\newcommand{\mdp}{\mathcal{M}}
%\newcommand{\Mdp}[1][]{\ensuremath{\mdp{#1}=(S{#1},I{#1},\Act,\pmdp{#1})}}
\newcommand{\MdpInit}[1][]{\ensuremath{\mdp{#1}=(S{#1},\,\sinit{#1},\,\Act,\,\probmdp{#1})}}
\newcommand{\probmdp}{\mathcal{P}}
\newcommand{\functions}[1][]{\ensuremath{\mathbb{Q}_{#1}}}
\newcommand{\poly}[1][]{\ensuremath{\mathbb{Q}[#1]}}

%\newcommand{\rew}{\ensuremath{\mathbb{E}}}
%\newcommand{\er}{\ensuremath{\mathrm{ER}}}
%\newcommand{\expRew}[2]{\ensuremath{\er^{#1}(\finally #2)}}
%\newcommand{\expRewT}[1][]{\ensuremath{\expRew{#1}{T}}}
%\newcommand{\expRewProp}[2]{\ensuremath{\rew_{\leq #1}(\finally #2)}}
%\newcommand{\expRewPropkT}{\ensuremath{\expRewProp{\kappa}{T}}}
%\newcommand{\rewFunction}{\ensuremath{\mathrm{rew}}}


%\newcommand{\ratfunceval}{\ensuremath{\ratfunc[{V\setminus\dom(u)}]}}
%\newcommand{\evalratfunc}[2]{\ensuremath{#1[{#2}/u]}}
%\newcommand{\Rloop}{\ensuremath{R_{\mathit{loop}}}}
%\newcommand{\Rout}{\ensuremath{R_{\mathit{out}}}}
\newcommand{\pol}{\ensuremath{g}}
\newcommand{\Par}{\ensuremath{{V}}}
\newcommand{\Expr}{\ensuremath{\mathsf{Expr}}}
\newcommand{\rat}[1]{\ensuremath{\Rationals_{#1}}}
%\newcommand{\poly}[1]{\ensuremath{\Integers_{#1}}}
\newcommand{\rdtmc}{\ensuremath{\mathcal{R}}}
\newcommand{\Rdtmc}[3]{\ensuremath{\rdtmc_{#1}^{#2}\llbracket #3\rrbracket}}
\newcommand{\pdtmc}{\ensuremath{\mathcal{P}}}
\newcommand{\AP}{\ensuremath{\mathit{AP}}}
\renewcommand{\Pr}{\ensuremath{\textnormal{Pr}}}
\newcommand{\Prr}[1]{\ensuremath{\Pr^{#1}}}
\newcommand{\sched}{\ensuremath{\sigma}}
\newcommand{\Sched}{\ensuremath{\mathit{Sched}}}

\newcommand{\rmdp}{\ensuremath{\mathfrak{R}}}
\newcommand{\Rmdp}[3]{\ensuremath{\mdp_{#1}^{#2}\llbracket #3\rrbracket}}
\newcommand{\Act}{\ensuremath{\mathit{Act}}}
\newcommand{\act}{\ensuremath{\alpha}}
\newcommand{\pmdp}{\ensuremath{\mathcal{P}}}

\newcommand{\pathset}{\mathsf{Paths}}
\newcommand{\paths}[2]{\pathset(#1,\allowbreak\,#2)}
\newcommand{\pathsfin}{\pathset_{\mathit{fin}}}
\newcommand{\pathsinf}{\pathset_{\mathit{inf}}}
%\newcommand{\path}{\pi}
\newcommand{\fpath}{\hat\pi}
\newcommand{\last}[1]{\mathit{last}(#1)}
\newcommand{\bad}{\ensuremath{\lightning}}
\newcommand{\undesired}{\ensuremath{\langle \bad \rangle}\xspace}
\newcommand{\sinklabel}{\mathpzc{sink}\xspace}
\newcommand{\sink}{\ensuremath{\langle \sinklabel \rangle}\xspace}
%\newcommand{\expandable}{\ensuremath{\langle \mathpzc{expandable}\rangle}\xspace}

\newcommand{\term}{\ensuremath{{\downarrow}}}
\newcommand{\expandable}{\ensuremath{{\uparrow}}}
\newcommand{\exit}{\ensuremath{{\downarrow}}}
\newcommand{\ExpRew}[2]{\ensuremath{\textnormal{\textsf{ExpRew}}^{#1}\left(#2\right)}}
\newcommand{\LExpRew}[2]{\ensuremath{\textnormal{\textsf{LExpRew}}^{#1}\left(#2\right)}}
\newcommand{\CExpRew}[3]{\ensuremath{\textnormal{\textsf{CExpRew}}^{#1}\left(#2\,|\,#3\right)}}
\newcommand{\CLExpRew}[3]{\ensuremath{\textnormal{\textsf{CLExpRew}}^{#1}\left(#2\,|\,#3\right)}}
%temporary mdp stuff
\newcommand{\Rewset}{\mathfrak C}
\newcommand{\Paths}{\mbox{\sl Paths}}

%% Math-Fonts
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\def\presuper#1#2%
  {\mathop{}%
   \mathopen{\vphantom{#2}}^{#1}%
   \kern-\scriptspace%
   #2}
   
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=.5pt] (char) {#1};}}


==> pics/packages.tex <==
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{mathtools}
%\usepackage{amsthm}
% \usepackage[pdfpagelabels=true,linktocpage]{hyperref}
\usepackage[usenames,dvipsnames]{color}
\usepackage{xcolor}
\usepackage{xspace}
\usepackage{microtype}
\usepackage{todonotes}
\usepackage{colonequals}
\usepackage{wasysym}
 \usepackage{booktabs}
\usepackage[affil-it]{authblk}



\usepackage{multirow}
\usepackage{multicol}

\usepackage{paralist}

\usepackage{subfigure}
\usepackage{url}
\usepackage{appendix}
\usepackage{graphicx}
\usepackage{float}
%\usepackage[pdfpagelabels=true]{hyperref}
\usepackage{algorithm}
\usepackage{listings}
%\usepackage{newalg}
\usepackage{nicefrac}
\usepackage{tikz} 
\usepackage{pgfplots}
%\usepgfplotslibrary{external}
%\pgfplotsset{compat=1.8}
%\tikzexternalize[prefix=TikzPictures/]
%\usepackage{marvosym}
\usepackage{wrapfig}




\lstset{
	basicstyle=\ttfamily,
    keywordstyle=\bfseries,
    showstringspaces=false,
    numbers=left,
    numberstyle=\tiny,
    morekeywords={}
}

\usetikzlibrary{arrows,decorations.pathmorphing,positioning,fit,trees,shapes,shadows,automata,calc} 
%\usetikzlibrary{patterns,arrows,arrows.meta,calc,shapes,shadows,decorations.pathmorphing,decorations.pathreplacing,automata,shapes.multipart,positioning,shapes.geometric,fit,circuits,trees,shapes.gates.logic.US,fit,automata,snakes,shapes.geometric}

\pagestyle{plain}

\tikzset{outline/.style args={#1}{%
  draw=#1,thick,fill=#1!50}}


==> pics/results_table.tex <==
\begin{tabular}[b]{@{}crrlrlrr@{}}
\toprule
Benchmark       & \#{}states & \#{}par     & specs      & \tool{MOSEK} (s)  & & Z3 \\
\midrule
BRP (pMC)   & $5382$   &  $2$    & $\er,\p,*$    & $23.17$ &($6.48$) & $-$                   \\
%	   & $28166$   &  $2$    & $\er,\p,*$    & $477.89$  &($73.88$) & $-$                  \\
   & $112646$   &  $2$    & $\er,\p,*$    & $3541.59$  &($463.74$) & $-$      \\
      & $112646$   &  $4$    & $\er,\p,*$    & $4173.33$  &($568.79$) & $-$              \\

  & $5382$   &  $2$    & $\er,\p$    & $3.61$   & &$904.11$                   \\
%  & $28166$   &  $2$    & $\er,\p$    & $52.105$  & &$\mathit{TO}$                  \\
  & $112646$   &  $2$    & $\er,\p$    & $479.08$  & &$\mathit{TO}$                  \\
  
NAND (pMC)  & $4122$   &  $2$    & $\er,\p,*$    & $14.67$ &($2.51$) & $-$                   \\
%  & $14322$   &  $2$    & $\er,\p,*$    & $80.92$ & ($13.91$) & $-$  \\
   & $35122$   &  $2$    & $\er,\p,*$    & $1182.41$ &($95.19$) & $-$                  \\
   & $4122$   &  $2$    & $\er,\p$    & $1.25$   && $1.14$                   \\
%   & $14322$   &  $2$    & $\er,\p$    & $9.81$  && $3.71$    \\
  & $35122$   &  $2$    & $\er,\p$    & $106.40$  && $11.49$                  \\
BRP (pMDP)   & $5466$   &  $2$    & $\er,\p,*$    & $31.04$ &($8.11$) & $-$                   \\      
%   & $28366$   &  $2$    & $\er,\p,*$    & $583.94$  &($72.91$) & $-$                   \\    
   & $112846$   &  $2$    & $\er,\p,*$    & $4319.16$  &($512.20$) & $-$                   \\    
   & $5466$   &  $2$    & $\er,\p$    & $4.93$  && $1174.20$                   \\      
%   & $28366$   &  $2$    & $\er,\p$    & $61.17$   && $\mathit{TO}$                   \\    
   & $112846$   &  $2$    & $\er,\p$    & $711.50$   && $\mathit{TO}$                   \\  
CONS (pMDP)  & $4112$   &  $2$    & $\er,\p,*$    & $102.93$  &($1.14$) & $-$                   \\      
%   & $16400$   &  $2$    & $\er,\p,*$    & $1474.73$  &($18.19$) & $-$                   \\    
   & $65552$   &  $2$    & $\er,\p,*$    & $\mathit{TO}$  &&  $-$                   \\    
   & $4112$   &  $2$    & $\er,\p$    & $6.13$   && $\mathit{TO}$                   \\      
%   & $16400$   &  $2$    & $\er,\p$    & $94.19$   && $\mathit{TO}$                   \\    
   & $65552$   &  $2$    & $\er,\p$    & $1361.96$  & & $\mathit{TO}$                   \\  
\bottomrule\end{tabular}

